A NUMA-Aware Provably-Efficient Task-Parallel Platform Based on the Work-First Principle

Task parallelism is designed to simplify the task of parallel programming. When executing a task parallel program on modern NUMA architectures, it can fail to scale due to the phenomenon called work inflation, where the overall processing time that multiple cores spend on doing useful work is higher compared to the time required to do the same amount of work on one core, due to effects experienced only during parallel executions such as additional cache misses, remote memory accesses, and memory bandwidth issues. It's possible to mitigate work inflation by co-locating the computation with the data, but this is nontrivial to do with task parallel programs. First, by design, the scheduling for task parallel programs is automated, giving the user little control over where the computation is performed. Second, the platforms tend to employ work stealing, which provides strong theoretical guarantees, but its randomized protocol for load balancing does not discern between work items that are far away versus ones that are closer. In this work, we propose NUMA-WS, a NUMA-aware task parallel platform engineering based on the work-first principle. By abiding by the work-first principle, we are able to obtain a platform that is work efficient, provides the same theoretical guarantees as the classic work stealing scheduler, and mitigates work inflation. Furthermore, we implemented a prototype platform by modifying Intel's Cilk Plus runtime system and empirically demonstrate that the resulting system is work efficient and scalable.

==> Makefile <==
# Standard Makefile for compiling LaTeX documents in the Supertech
# group.

DOC=locality

# This line is intentionally blank.

TARGETS=$(patsubst %,%.pdf,$(DOC))

OTHERS = code-*.tex figures/*.tex figures/cropped/*.pdf Makefile supertech-acm.sty allpapers.bib

DEPS_DIR = .deps

INCLUDE_DIR=.

LATEXMK = TEXINPUTS=$(INCLUDE_DIR)/: BIBINPUTS=$(INCLUDE_DIR)/: BSTINPUTS=$(INCLUDE_DIR)/: latexmk
LATEXMK_FLAGS = -pdflatex="pdflatex --shell-escape %O %S" -pdf -dvi- -ps- -recorder -M -MP \
                  -e 'show_cus_dep();' \

default: pdf
.PHONY:  pdf default all remake clean allclean

all: $(TARGETS)

-include $(DEPS_DIR)/$(DOC).pdfP

ifneq (,$(findstring B,$(MAKEFLAGS)))
LATEXMK_FLAGS += -gg
endif

$(DEPS_DIR) :
	if [ ! -d $(DEPS_DIR) ]; then mkdir $@; fi

$(DOC).pdf : $(OTHERS)

###########################################################################
## Make targets for cleaning

clean%:
	rm -f $*.aux $*.ps $*.pdf $*.dvi $*.bbl $*.blg $*.tmp $*.lof $*.log $*.toc $*.out $*.fls $*.fdb_latexmk $(DEPS_DIR)/$*.pdfP *~ *.tex.bak

clean: clean$(DOC)

allclean:
	rm -f *.aux *.dvi *.bbl *.blg *.tmp *.lof *.log *.toc *.out *.fls *.fdb_latexmk $(DEPS_DIR)/*.pdfP $(DOC).pdf *~



###########################################################################
## Make targets for document

pdf : $(DOC).pdf

$(DOC).pdf : $(DOC).tex $(OTHERS)
	if [ ! -e $(DEPS_DIR) ]; then mkdir $(DEPS_DIR); fi
	$(LATEXMK) $(LATEXMK_FLAGS) -MF $(DEPS_DIR)/$@P $<
	if [ -e $@ ]; then touch $@; fi

# Some nonsense that latexmk doesn't understand with minted can be fixed by telling that these rules are easy.
%.w18 %.out.pyg %.aex: %.tex
	@echo > /dev/null
# remake :
# 	if [ ! -e $(DEPS_DIR) ]; then mkdir $(DEPS_DIR); fi
# 	$(LATEXMK) -g -deps-out=$(DEPS_DIR)/$(DOC).pdfP $(DOC).tex
# 	if [ -e $(DOC).pdf ]; then touch $(DOC).pdf; fi


==> cut.tex <==
%% --------------------------------------------------------
%% Rework of numaws 
%% --------------------------------------------------------

\begin{wrapfigure}{R}{0.5\columnwidth}
%\begin{figure}
\center
\includegraphics[width=1.5in]{figures/cropped/zlayout_fine.pdf}\\
\vspace{0.1in}
\includegraphics[width=1.5in]{figures/cropped/zlayout.pdf}
\caption{The first matrix shows the standard Z-Morton layout where every
element lies on the curve. The second matrix shows the blocked Z-Morton layout, 
where the blocks are laid out in the Z order, and data within each block is laid out in row-major
order.}
\label{fig:morton}
%\end{figure}
\end{wrapfigure}

%% --------------------------------------------------------
%% Rework of motivate 
%% --------------------------------------------------------

%% benefit of work-first re-written, incorporated into scheduling part
\paragraph{Work-stealing scheduler.} In work stealing, each \defn{worker}
thread (a surrogate of a processing core) maintains a \defn{deque} (a double
ended queue) of work items.  Most of the time, each worker operates on its own
deque locally and communicates with one another only when it runs out of work
to do, i.e., its deque has become empty.  When that happens, a worker turns
into a \defn{thief} and \emph{randomly} chooses another worker, the
\defn{victim}, to steal work from.  A worker always operates on its own local
deque like a stack in a first-in-first-out fashion, but steals from the top of
a victim's deque, taking the oldest work.

What gets pushed onto the deque depends on the implementation.  Cilk Plus
implements \defn{work-first} (also called \defn{continuation-stealing}),
meaning that upon a spawn, the \emph{continuation} of the spawning parent gets
pushed onto the deque, and the worker encountering the spawn continues to
execute the spawned child.  In the literature, people have also proposed
\defn{help-first}~\cite{GuoBaRa09} (also called \defn{child-stealing}), which
does the opposite --- push the packaged spawned child onto the deque and
execute the continuation of the parent.  In help-first, only when the spawning
parent executes a sync, the worker then tries to pop off and execute the 
packaged spawned children.

Regardless of which mechanism a platform implements, upon a \spawn, something
has to be pushed onto the deque in order to enable parallel execution.  Such
an overhead, referred to as the \defn{spawn overhead}, is difficult to avoid
entirely.  However, work-first does have some advantages over help-first.  For
one, work-first can be more space efficient.  In help-first, all the spawned
children must be packaged up and pushed onto the deque even in single-core
execution; in work-first in constrast, if the continuation of the parent is
not stolen, once the previous spawned child return, the next spawned child
reuses the same stack space.  For two, with work-first, execution of a worker
between successful steals mirrors exactly that of a serial elision, and thus
has similar cache behavior (for private caches) with respect to serial
elision.  Thus, one can optimize the cache behavior of parallel code by
optimizing that of the serial elision.

%% --------------------------------------------------------

%% benefit of work-first
Even though work-first principle does not dictate the choice of work-first
versus help-first, Cilk Plus implements work-first because of its multiple 
benefits over help-first.  First, it allows the workers to get to work sooner 
than later. \jnote{Reword}  Imagine the following code snippet: 
%
\begin{quote} 
\small
\begin{verbatim}
for(int i=0; i < 1000; i++) {
    cilk_spawn foo(i);
}
cilk_sync;
\end{verbatim}
\end{quote} 
%
With help-first, a worker would not execute any \texttt{foo(i)} call
until it encounters \sync.  Instead, it would first create $1000$ packaged 
spawned \texttt{foo(i)} before executing any of it.  In contrast,
work-first would simply push the continuation of the parent onto the deque
and execute the next \texttt{foo(i)}.  Second, relatedly, help-first is also 
less space efficient compared to work-first, since in help-first 
a worker must package the $1000$ spawned calls and push them onto the deque, as
opposed to push the continuation of the parent, which allows the worker to reuse 
the space.  Third, and most importantly, work-first allows the one-core 
execution to mirror exactly that of a serial elision, and help-first does not.  
Finally, related to the third point, one can bound the extra cache misses during
parallel execution (for private caches) using work-first, since the cache misses 
are bounded with respect to the serial execution.

%% --------------------------------------------------------
%% Rework of intro 
%% --------------------------------------------------------

In work stealing, worker threads (surrogates of processing cores) load balance
by ``stealing'' work when necessary.  The additional cache misses (for private
caches) due to parallel execution are directly correlated with the number of
successful steals occurred during parallel execution, which is upper bounded
by $O(P\spa)$.  \NUMAWS maintains the same theoretical bound, albeit with a
larger constant hidden in the big-$O$.

Assuming the comptuation contains sufficient \defn{parallelism}, defined
precisely as $\work / \spa$ (i.e., average amount of work along each step of
the longest sequential dependences), this bound states that the parallel
execution time should be dominated by the $\work / P$ term.  In the absence of
work inflation, a computation with ample parallelism should exhibit near
linear speedup.

%% --------------------------------------------------------
%% abstract 
%% --------------------------------------------------------

In this work, we show that it is possible to engineer a NUMA-aware provably
efficient task parallel platform using a modified work stealing algorithm that
retains the same nice theoretical guarantees while mitigating work inflation.
Specifically, we proposes a variant of a work stealing algorithm that employs
a randomzied locality-biased steal protocol with lazy work pushing that
provides the same asymptotic guarantees as the classic work stealing
algorithm.  Since one must co-locate computation with data in the same NUMA
domain (i.e., a socket) in order to minimize remote memory accesses, our
platform also provides a simple API to allow the programmer to specify
locality hints and transform data layout in a way that allows the data and
computation to be co-located.  Crutially, the engineering of our platform
abides by a principle referred to as the \defn{work-first principle} proposed
by Frigo et. al, which states that one should minimize the scheduling overhead
borne by the work of the computation, and instead move the overhead onto the
span.  

%% --------------------------------------------------------
%% NUMAWS 
%% --------------------------------------------------------

In the implementation, the locality hint is carried around in the 
shadow frame of a Cilk function (defined in \secref{motivation}).  When a function
$F$ spawns $G$, in which virtual place $G$ should execute is dictated by the
locality hint stored in $F$'s shadow frame.  Moreover, $G$ also inherits that
locality hint.  That means, to translate the locality hints specified, the
code shown in \figref{sort} is compiled into code shown in \figref{sortcomp},
where the \texttt{\_\_set\_locality} is a runtime call updating the locality 
hint in the current function's shadow frame. 

%% STOPPED HERE

With locality-biased steals, a worker can still end up with work earmarked for
a remote socket.  The lazy work-pushing is designed to correct that ---
pushing the work back to the socket that it is earmarked for, but do so in
a lazy fashion.


\anote{Note the off by one and mention work-first and how top level function
must be called.}
Because Cilk Plus performs work-first, such locality hints actually translates
to updating the locality 

\begin{figure}
\footnotesize
\begin{codebox}
\Procname{$\proc{MergeSortTop}$(int *$in$, int *$tmp$, int $n$)}
\li $\cdots$ \Comment{Base case in-place sort}
\li \Else
\li   \_\_set\_locality(p1);
\li   cilk\_spawn $\proc{MergeSort}$($in$, $tmp$, $n/4$) \Comment{@ p0}
\li   \_\_set\_locality(p2);
\li   cilk\_spawn $\proc{MergeSort}$($in$ + $n/4$, $tmp$ + $n/4$, $n/4$) \Comment{@ p1}
\li   \_\_set\_locality(p3);
\li   cilk\_spawn $\proc{MergeSort}$($in$ + $n/2$, $tmp$ + $n/2$, $n/4$) \Comment{@ p2}
\li   \_\_set\_locality(ANY);
\li   $\proc{MergeSort}$($in$ + $3n/4$, $tmp$ + $3n/4$, $n$ - $3n/4$) \Comment{@ p3}
\li   \_\_set\_locality(p0);
\li   cilk\_sync;
\li   $\cdots$ \Comment{Rest compiled similarly}
% \li   int *$tmp1$ = $tmp$, *$tmp2$ = $tmp$ + $n/2$;
% \li   \_\_set\_locality(p2);
% \li   cilk\_spawn $\proc{ParMerge}$($in$, $in$ + $n/4$, $n/4$, $n/4$, $tmp1$); \Comment{@ p0}
% \li   \_\_set\_locality(ANY);
% \li   $\proc{ParMerge}$($in$ + $n/2$, $in$ + $3n/4$, $n/4$, $n$ - $3n/4$, $tmp2$); \Comment{@ p2}
% \li   cilk\_sync;
% \li   $\proc{ParMerge}$($tmp1$, $tmp2$, $n/2$, $n$ - $n/2$, $in$); @ ANY 
    \End 
\end{codebox}
\vspace{-2mm}
\caption{Conceptually how the locality hints shown in \figref{sort} are
compiled.}
\label{fig:sortcomp}
\end{figure}

Specifically, if when $F$ spawns $G$, the spawning of $G$ is marked with
locality for virtual place $i$, the shadow frame for $G$ will store this
locality information throughout its life time.  

%% --------------------------------------------------------

the runtime data structures
In the implementation, the locality hint is carried 
around in the shadow frame of a Cilk function (defined in \secref{motivation}).

%% --------------------------------------------------------

\begin{figure}
\footnotesize
\begin{codebox}
\Procname{$\proc{MergeSortTop}$(int *$in$, int *$tmp$, int $n$)}
\li \If $n <$ BASE\_CASE
\li \Then in\_place\_qsort(in, n)
\li \Else
\li     \_\_cilkrts\_update\_locality(1);
\li     cilk\_spawn $\proc{MergeSort}(in, tmp, n/4)$
\li     \_\_cilkrts\_update\_locality(2);
\li     cilk\_spawn $\proc{MergeSort}(in+n/4, tmp+n/4, n/4)$
\li     \_\_cilkrts\_update\_locality(3);
\li     cilk\_spawn $\proc{MergeSort}(in+n/2, tmp+n/2, n/4)$
\li     \_\_cilkrts\_unset\_locality();
\li                $\proc{MergeSort}(in+n/2, tmp+n/2, n/4)$
\li     \_\_cilkrts\_update\_locality(3);
\li     cilk\_sync;
    \End
\end{codebox}
\caption{Pseudocode for the top-level function for parallel mergesort
with locality hint.}
\label{fig:sort}
\end{figure}

\figref{sort} shows an example of the API.  

%% --------------------------------------------------------
%% Motivation 
%% --------------------------------------------------------

the stolen frame is then promoted into a
\defn{full frame}, which contains more bookkeeping information that the
runtime uses to keep track of parallel executions.  In this example, if $F$ is
stolen for the first time (which is only possible after it spawns), the thief
resumes $F$ at the continuation, executing it concurrently with $G$ executing
on the victim.  

Whenever a function
$F$ spawns another function $G$, $F$'s continuation becomes \defn{stealable},
accomplished by pushing $F$'s shadow frame onto the worker's deque, and the
frame contains enough information to resume the execution at the continuation.

Whenever a frame is stolen successfully for the first time, \emph{actual} parallelism is 
realized, and the stolen frame is then promoted into a
\defn{full frame}, which contains more bookkeeping information that the
runtime uses to keep track of parallel executions.  In this example, if $F$ is
stolen for the first time (which is only possible after it spawns), the thief
resumes $F$ at the continuation, executing it concurrently with $G$ executing
on the victim.  For the convenience of bookkeeping, the thief also leaves a
full frame on top of the victim's deque (conceptually representing $G$).  

In short, the runtime maintains two different types of frames: the full frames
and the shadow frames, with the following invariants.  1)  

%% --------------------------------------------------------

\NUMAWS extends the classic work-stealing scheduler in Cilk Plus to
incorporate the following mechanisms to mitigate NUMA effects: locality-biased 
steals, lazy work pushing, and a simple data layout transformation that is 
applied only to a subset of benchmarks.  This section describes these extensions 
in detail and argues why the modifications still allows for the same 
theoretical bounds.  

%% --------------------------------------------------------

Historically, different Cilk dialects have all implemented the classic work
stealing algorithm with its engineering centered around the work-first
principle.  These implementations have demosntrated the effectiveness of the
principle.  Frigo et.\@ al~\cite{FrigoLeRa98} hae demonstrated that Cilk-5
incurs little scheduling overhead, and its design of the ``THE protocol'' that
synchronizes between a thief and a vicitm and the ``two-clone'' compilation
strategies both embody the work-first principle.  Perhaps more telling is the
Cilk-M example: in Cilk-M~\cite{LeeBoHu10}, Lee et.\@ al employs a
heavy-weight system call to maintain the ``cactus stack'' abstraction during
parallel execution in order to provide interoperability with legacy C binary.
Despite the use of a heavy-weight system call, since the system call is
invoked only up on a successful steal, Cilk-M performed comparably to the
original Cilk-5 and Intel's Cilk Plus implementations.

%% --------------------------------------------------------

Throughout the paper, we shall use the 
keywords \spawn and \sync to describe how task parallelism works, but
note that many concurrency platforms have similar constructs to implement
task parallelism though with slightly different syntax.  Paralleism can be
create using the keyword \spawn.  When a function $F$ \defn{spawns} another
function $G$ (invoking $G$ with the keyword \spawn), the continuation of $F$
may potentially execute in parallel with $G$.  The keyword \sync specifies
that control cannot pass beyond the \sync statement until all previously
spawned children within the enclosing function has returned.

%% --------------------------------------------------------
%% Intro 
%% -------------------------------------------------------- %

The rest of the paper is organized as follows.  \secref{motivation} examines the 
implementation of Intel Cilk Plus, the system that \NUMAWS is based on.  We show 
that Cilk Plus is work efficient and follows the work-first principle, but can 
fail to scale due to work inflation.  \secrefs{numaws}{eval} present the
system, its analysis, and evaluation.  Finally, \secref{related} disccusses  
prior work on NUMA-aware task parallel platforms and why they failed to satisfy 
our desired goals.  

%% -------------------------------------------------------- %

In work stealing, each worker thread (i.e., a surrogate of a processing core)
maintains a \defn{deque} (a double ended queue) of work items.  Each worker
operates on its own deque locally for the most part, and communicates with one
another only when it runs out of work to do, i.e., its deque has become empty.
When that happens, a worker turns into a \defn{thief} and \emph{randomly}
chooses another worker, the \defn{victim}, to steal work from.  In \NUMAWS,
locality-biased steals simply change the probability distribution of how a
worker steals to preferentailly biase the worker to take work from its local
socket over ones from the remote sockets.  With locality-biased steals, a
worker can still end up with work items that originate from a remote socket.
The lazy work-pushing is designed to correct that --- pushing the work items
back to the socket that it came from --- but do so in a lazy fashion.

In practice, work stealing has also been demonstrated to incur low scheduling
overhread~\cite{FrigoLeRa98}.  Crutially, as informed by the theory, a work
stealing scheduler can be implemented efficiently by following the
\defn{work-first principle}~\cite{FrigoLeRa98}, which states that one should
minimize the overhead borne by the work term ($\work$) and move the overhead
onto the span term ($\spa$).  Intuitively, a scheduler necessarily needs to
incur scheduling overhead due to the extra bookkeeping necessary to enable
correct parallel execution.  Within the context of a work-stealing scheduler,
the work-first principle states that it's best to incur such scheduling
overhead on the control path that can be amortized against successful steals;
put it differently, whenever a choice can be made to incur overhead on a thief
stealing versus on a worker busy working, it's always perferred to incur the
overhead on the thief stealing.  

Why such a choice leads to better performance and can be understood in two
ways.  First, the parallelism of an applicaiton is defined as $\work/\spa$,
which can be thought of as how much work is there along each step of the span.
Assuming the application contains ample parallelism (i.e., $\work/\spa \gg
P$), the execution time is dominated by the $\work / P$ term, and thus it's
better to incur overhead on the $\spa$ term.  Second, in practice, when the
applicaiton contains ample parallelism, steals occur infrequently.
 
Historically, different Cilk dialects have all implemented the classic work
stealing algorithm with its engineering centered around the work-first
principle.  These implementations have demosntrated the effectiveness of the
principle.  Frigo et.\@ al~\cite{FrigoLeRa98} hae demonstrated that Cilk-5
incurs little scheduling overhead, and its design of the ``THE protocol'' that
synchronizes between a thief and a vicitm and the ``two-clone'' compilation
strategies both embody the work-first principle.  Perhaps more telling is the
Cilk-M example: in Cilk-M~\cite{LeeBoHu10}, Lee et.\@ al employs a
heavy-weight system call to maintain the ``cactus stack'' abstraction during
parallel execution in order to provide interoperability with legacy C binary.
Despite the use of a heavy-weight system call, since the system call is
invoked only up on a successful steal, Cilk-M performed comparably to the
original Cilk-5 and Intel's Cilk Plus implementations.

%--------------------------------------------------------

\NUMAWS employs a variant of work stealing that extends the classic algorithm
with two mechanisms to mitigate NUMA effects: \defn{locality-biased steals},
and \defn{lazy work-pushing}.  In work stealing, each worker thread (i.e., a
surrogate of a processing core) maintains a \defn{deque} (a double ended
queue) of work items.  Each worker operates on its own deque locally for the
most part, and communicates with one another only when it runs out of work to
do, i.e., its deque has become empty.  When that happens, a worker turns into
a \defn{thief} and \emph{randomly} chooses another worker, the \defn{victim},
to steal work from.  In \NUMAWS, locality-biased steals simply change the
probability distribution of how a worker steals to preferentailly biase the
worker to take work from its local socket over ones from the remote sockets.
With locality-biased steals, a worker can still end up with work items that
originate from a remote socket.  The lazy work-pushing is designed to correct
that --- pushing the work items back to the socket that it came from --- but
do so in a lazy fashion.

%% --------------------------------------------------------

Critically, the engineering of our scheduler abides by a principle referred 
to as the \defn{work-first principle}~\cite{FrigoLeRa98}, which states that 
one should minimize the overhead borne by the work term ($\work$) and move the 
overhead onto the span term ($\spa$), then the resulting scheduler should be 
efficient.  Intuitively, a scheduler necessarily needs to
incur scheduling overhead due to the extra bookkeeping necessary to enable
correct parallel execution.  Within the context of a work-stealing scheduler,
the work-first principle states that it's best to incur such scheduling
overhead on the control path that can be amortized against successful steals;
put it differently, whenever a choice can be made to incur overhead on a thief
stealing versus on a worker busy working, it's always perferred to incur the
overhead on the thief stealing. 

% Note that the original work stealing scheduler, when implemented efficiently, 
% provides all aforementioned properties except for Property \ref{prop:numa}.

As informed by theory, if one implements work stealing in a way that abide by 
the \defn{work-first principle}~\cite{FrigoLeRa98}, which states that one should
minimize the overhead borne by the work term ($\work$) and move the overhead
onto the span term ($\spa$), then the resulting scheduler should be 
efficient.  Specifically, the scheduler should be both \defn{work-efficient}, i.e., 
when going from 
little time is spent on scheduling when executing
the computation assuming the comptuation contains sufficient parallelism.
Here, one can define \defn{parallelism} precisely: 
$\work / \spa$ (i.e., average amount of work along each step of the
longest sequential dependences).  

%% --------------------------------------------------------

that it's possible to modify work stealing in a principled way, so that the
resulting scheduler is NUMA-aware, and still retain its original nice
properties.  Specificially, we propose two simple mechanisms to aid
NUMA-awareness: \defn{locality-based randomized stealing} and \defn{lazy work
pushing}, which results a scheduler with the following properties: 
%
\begin{enumerate}
\item It retains the classic work stealing's nice theoretical guarantees; 
        \label{prop:provable}
\item It is \defn{work efficient}, namely, the scheduler does not incur
unnecessary scheduling overhead that causes the one-worker execution time
to increase. \label{prop:workeff}
\item It incurs low parallel scheduling overhead --- when the application
contains sufficient parallelism, little time is spent in the scheduler; and
\label{prop:scale}
\item It mitigates work inflation.  \label{prop:numa}
\end{enumerate}

%% --------------------------------------------------------

A crutial aspect of work stealing is how it performs work distribution and
load balancing: it utilizes a randomized distributed protocol.  At a
high-level, each worker thread (which serves as a surrogate of a processing
core) maintains a \defn{deque} (a double ended queue) of work items.  Each
worker operates on its own deque locally for the most part, and communicates
with one another only when it runs out of work to do, i.e., its deque has
become empty.  When that happens, a worker turns into a \defn{thief} and
\emph{randomly} chooses another worker, the \defn{victim}, to steal work from.
This randomized stealing is essential to efficient load balacing --- the
randomization allows the scheduler to both bound the amount of contentions one
may incur on a worker's deque and the extra scheduling overhead due to failed
steal attempts during load balancing, thereby allowing for provably efficient
execution time.  Moreover, randomization also allows one to bound the number
of successful steals, which then in turn bounds the stack space consumption
and additional cache misses with respect to serial execution.  

Even though the randomized distributed protocol leads to many nice properties,
the randomized strategy for load balancing seems to be directly at odds with
obtaining scalable performance for NUMA architectures, because it does not
discern between work items that are far away versus ones that are closer and
give user little control over where the computation is scheduled.

%% --------------------------------------------------------

The nice abstraction provided by task parallelism can be a double-edged
sword, however: the scheduling is automated, but it also removes the
programmer out of the loop entirely, and the programmer has little control
over where the computation is scheduled.  The lack of control can be
especially problematic for modern parallel systems with shared memory.  In
order to provide the shared-memory abstraction with sufficient memory
capacity, modern parallel systems often employ deep memory hierarchies with
Non-Uniform Memory Accesse (NUMA) behaviors, in which the latency of a memory
access can differ drastically, ranging from a few cycles to hundreds of
cycles, depending on where the memory access is serviced.  Consequently, a
major performance bottleneck in task parallel computations is
\defn{work inflation}~\cite{OlivierDeSuSc12}, where the overall processing
time executing on multiple cores increases compared to that on one core, due
to effects experienced only during parallel executions such as additional
cache misses, remote memory accesses, and memory bandwidth issues.  With work
inflation, a task parallel computation can fail to scale, despite the
computation spends little time in scheduling.

%% --------------------------------------------------------

The nice abstraction provided by task parallelism can be a double-edged
sword, however: the scheduling is automated, but it also removes the
programmer out of the loop entirely, and the programmer has little control
over where the computation is scheduled.  The lack of control can be
especially problematic for modern parallel systems with shared memory.  In
order to provide the shared-memory abstraction with sufficient memory
capacity, modern parallel systems often employ deep memory hierarchies with
Non-Uniform Memory Accesse (NUMA) behaviors, in which the latency of a memory
access can differ drastically, ranging from a few cycles to hundreds of
cycles, depending on where the memory access is serviced.  Consequently, a
major performance bottleneck in task parallel computations is
\defn{work inflation}~\cite{OlivierDeSuSc12}, where the overall processing
time executing on multiple cores increases compared to that on one core, due
to effects experienced only during parallel executions such as additional
cache misses, remote memory accesses, and memory bandwidth issues.  With work
inflation, a task parallel computation can fail to scale, despite the
computation spends little time in scheduling.

Most concurrency platforms, including all the aforementioned ones, schedule 
task parallel computations using work stealing~\cite{BlumofeLe94,
BlumofeLe99,AroraBlPl98,AroraBlPl01}, which in its classic forms, 
enjoys many theoretical guarantees --- it provides asymptotically optimal execution
time~\cite{BlumofeLe94,BlumofeLe99,AroraBlPl98,AroraBlPl01}; it uses bounded
stack space during parallel execution~\cite{BlumofeLe99}; and it allows for
good cache locality with respect to sequential execution when using private
caches~\cite{AcarBlBl02}.  




==> figures/breakdown.tex <==
\usetikzlibrary{patterns}
\newcounter{groupcount}
\pgfplotsset{
    draw group line/.style n args={5}{
        after end axis/.append code={
            \setcounter{groupcount}{0}
            \pgfplotstableforeachcolumnelement{#1}\of\datatable\as\cell{%
                \def\temp{#2}
                \ifx\temp\cell
                    \ifnum\thegroupcount=0
                        \stepcounter{groupcount}
                        \pgfplotstablegetelem{\pgfplotstablerow}{X}\of\datatable
                        \coordinate [yshift=#4] (startgroup) at (axis cs:\pgfplotsretval,0);
                    \else
                        \pgfplotstablegetelem{\pgfplotstablerow}{X}\of\datatable
                        \coordinate [yshift=#4] (endgroup) at (axis cs:\pgfplotsretval,0);
                    \fi
                \else
                    \ifnum\thegroupcount=1
                        \setcounter{groupcount}{0}
                        \draw [
                            shorten >=-#5,
                            shorten <=-#5
                        ] (startgroup) -- node [anchor=base, yshift=0.5ex] {#3} (endgroup);
                    \fi
                \fi
            }
            \ifnum\thegroupcount=1
                        \setcounter{groupcount}{0}
                        \draw [
                            shorten >=-#5,
                            shorten <=-#5
                        ] (startgroup) -- node [anchor=base, yshift=0.5ex] {#3} (endgroup);
            \fi
        }
    }
}

\selectcolormodel{gray}
\begin{tikzpicture}
\pgfplotstableread{
X	Gp	CleanVanilla	ModifiedVanilla	CleanLocality	ModifiedLocality
1	Cilksort	1.00	0.00	1.02	0.82
2	Heat	1.00	0.04	0.99	0.03
3	Strassen	1.00	0.63	0.99	0.63
4	Lu	1.00	0.91	0.99	0.93
5	hull1	1.00	0.00	0.99	0.85
6	hull2	1.00	0.00	1.01	0.64
7	cg	1.00	0.00	1.03	0.52
}\datatable

\begin{axis}[
    axis lines*=left, ymajorgrids,
    ymin=0,
    ybar,
    bar width=8pt,
    width=6.5in,
    height=4in,
    legend columns=4,
    xtick=data,
    xticklabels from table={\datatable}{Gp},
    xticklabel style={xshift=-0.3ex,anchor=north},
   legend style={at={(0.5,1)},anchor=north}
]

\addplot [postaction={pattern=north east lines}] table [x=X, y=CleanVanilla] {\datatable};\addlegendentry{Vanilla}
\addplot  table [x=X, y=CleanLocality] {\datatable}; \addlegendentry{Clean on  Locality}
\addplot table [x=X, y=ModifiedLocality] {\datatable}; \addlegendentry{Locality}
\addplot  [postaction={pattern=horizontal lines}] table [x=X, y=ModifiedVanilla] {\datatable}; \addlegendentry{Z Layout on Vanilla}
\end{axis}
\end{tikzpicture}


==> figures/effects-overview.tex <==
\selectcolormodel{gray}
\begin{tikzpicture}[scale=1]
\pgfplotstableread{
X	Gp	none	zlayout	bias	push
1	cilksort	1.00	0	0.77	0.76
2	heat	1.00	0.05	0.05	0.04
3	lu	1.00	1.00	0.99	0.99
4	strassen	1.00	1.01	0.99	1.00
5	hull1	1.00	0	1.03	0.86
6	hull2	1.00	0	1.01	0.63
7	cg	1.00	0	1.00	0.50
8	fft	1.00	0.00	1.11	0.95
}\datatable

\begin{axis}[
    axis lines*=left, ymajorgrids,
    ybar,
    ymin=0,
    bar width=9pt,
    width=\textwidth,
    height=1.5in,
    xtick=data,
    xticklabels from table={\datatable}{Gp},
    xticklabel style={font=\large,align=center},
    yticklabel style={font=\large},
     legend style={at={(0,-0.5)},anchor=west, legend columns=4}
]

\addplot table [x=X, y=none, ] {\datatable}; \addlegendentry{None}
\addplot table [x=X, y=zlayout] {\datatable}; \addlegendentry{Z Layout}
\addplot table [x=X, y=bias] {\datatable}; \addlegendentry{Biased Stealing}
\addplot table [x=X, y=push] {\datatable}; \addlegendentry{Work Pushing}

\end{axis}
\end{tikzpicture}

==> figures/scalability-all.tex <==
%\selectcolormodel{gray}
\begin{tikzpicture}[scale=0.60]
\pgfplotstableread{
X	cg	cilksort	heat	hull1	hull2 	lu	strassen	strassenz	fft	matmul	matmulz
1.0	1.0	1.0	1.0	1.0	1.0	1.0	1.0	1.0	1.0	1.0	1.0
8.0	7.1	5.0	1.6	5.2	6.7	8.0	6.1	6.5	6.6	7.6	8.0
16.0	13.6	14.6	3.5	5.4	11.7	15.4	11.6	12.4	8.2	15.2	15.9
24.0	19.7	19.1	5.1	6.7	15.5	22.3	16.9	18.2	8.8	22.7	23.7
32.0	25.8	26.6	11.4	9.0	21.3	29.8	22.4	23.6	16.4	29.8	31.3
}\datatable

\begin{axis}[
    axis lines*=left, ymajorgrids,
    every axis plot/.append style={ultra thick},
    xlabel=\# of Cores ($P$),
    ylabel=Scalability ($T_1$/$T_P$),
    legend columns=2, 
    ymin=0,
    xtick=data,
    legend style={at={(0.03,1.0)},anchor=west}
]

\addplot [width=5mm] table [x=X,y=cilksort]{\datatable};\addlegendentry{Cilksort}
\addplot table [x=X,y=heat]{\datatable};\addlegendentry{Heat}
\addplot table [x=X,y=strassen]{\datatable};\addlegendentry{Strassen}
\addplot table [x=X,y=strassenz]{\datatable};\addlegendentry{Strassen Z}
\addplot table [x=X,y=lu]{\datatable};\addlegendentry{Lu}
\addplot table [x=X,y=hull1]{\datatable};\addlegendentry{Hull1}
\addplot table [x=X,y=hull2]{\datatable};\addlegendentry{Hull2}
\addplot table [x=X,y=cg]{\datatable};\addlegendentry{cg}
\addplot table [x=X,y=fft]{\datatable};\addlegendentry{fft}
\addplot table [x=X,y=matmul]{\datatable};\addlegendentry{Matmul}
\addplot table [x=X,y=matmul]{\datatable};\addlegendentry{Matmul Z}
\end{axis}
\end{tikzpicture}


==> figures/scalability4way.tex <==
%\selectcolormodel{gray}
\begin{tikzpicture}
\pgfplotstableread{
X	cg	Cilksort	Heat	Hull1	Hull2	Lu	Strassen
1.0	1.0	1.0	1.0	1.0	1.0	1.0	1.0
8.0	7.6	7.9	8.2	4.6	7.3	7.8	7.5
16.0	14.5	15.2	16.0	7.1	13.5	15.2	14.5
24.0	20.5	21.1	23.4	8.6	18.2	22.2	20.7
32.0	25.1	26.6	30.3	9.0	21.3	29.8	26.0
}\datatable

\begin{axis}[
    axis lines*=left, ymajorgrids,
    every axis plot/.append style={ultra thick},
    xlabel=\# of Cores ($P$),
    ylabel=Scalability ($T_1$/$T_P$),
    ymin=0,
    xtick=data,
    legend style={at={(0.03,0.7)},anchor=west}
]

\addplot [width=5mm] table [x=X,y=Cilksort]{\datatable};\addlegendentry{Cilksort}
\addplot table [x=X,y=Heat]{\datatable};\addlegendentry{Heat}
\addplot table [x=X,y=Strassen]{\datatable};\addlegendentry{Strassen}
\addplot table [x=X,y=Lu]{\datatable};\addlegendentry{Lu}
\addplot table [x=X,y=Hull1]{\datatable};\addlegendentry{Hull1}
\addplot table [x=X,y=Hull2]{\datatable};\addlegendentry{Hull2}
\addplot table [x=X,y=cg]{\datatable};\addlegendentry{cg}
\end{axis}
\end{tikzpicture}


==> figures/work-inf.tex <==
\usepackage{pgfplots, pgfplotstable}

\pgfplotsset{
    draw group line/.style n args={5}{
        after end axis/.append code={
            \setcounter{groupcount}{0}
            \pgfplotstableforeachcolumnelement{#1}\of\datatable\as\cell{%
                \def\temp{#2}
                \ifx\temp\cell
                    \ifnum\thegroupcount=0
                        \stepcounter{groupcount}
                        \pgfplotstablegetelem{\pgfplotstablerow}{X}\of\datatable
                        \coordinate [yshift=#4] (startgroup) at (axis cs:\pgfplotsretval,0);
                    \else
                        \pgfplotstablegetelem{\pgfplotstablerow}{X}\of\datatable
                        \coordinate [yshift=#4] (endgroup) at (axis cs:\pgfplotsretval,0);
                    \fi
                \else
                    \ifnum\thegroupcount=1
                        \setcounter{groupcount}{0}
                        \draw [
                            shorten >=-#5,
                            shorten <=-#5
                        ] (startgroup) -- node [anchor=base, yshift=0.5ex] {#3} (endgroup);
                    \fi
                \fi
            }
            \ifnum\thegroupcount=1
                        \setcounter{groupcount}{0}
                        \draw [
                            shorten >=-#5,
                            shorten <=-#5
                        ] (startgroup) -- node [anchor=base, yshift=0.5ex] {#3} (endgroup);
            \fi
        }
    }
}

\begin{figure}[h!]
\begin{tikzpicture}
\pgfplotstableread{
X	Gp	Type	Cores	Scheduling	Work	Idle
1	Cilksort	CleanVanilla	T1	0.00	1.00	0.00
2	Cilksort	CleanVanilla	T32	0.02	2.06	0.01
3	Cilksort	ModifiedLocality	T1	0.00	0.17	0.00
4	Cilksort	ModifiedLocality	T32	0.00	0.20	0.00
5	Heat	CleanVanilla	T1	0.00	3.52	0.00
6	Heat	CleanVanilla	T32	0.06	23.51	0.22
7	Heat	ModifiedLocality	T1	0.00	3.04	0.00
8	Heat	ModifiedLocality	T32	0.07	3.07	0.80
9	Strassen	CleanVanilla	T1	0.00	1.08	0.00
10	Strassen	CleanVanilla	T32	0.01	1.55	0.28
11	Strassen	ModifiedLocality	T1	0.00	19.95	0.00
12	Strassen	ModifiedLocality	T32	0.67	28.40	0.12
13	Lu	CleanVanilla	T1	0.00	9.88	0.00
14	Lu	CleanVanilla	T32	0.10	11.72	0.21
15	Lu	ModifiedLocality	T1	0.00	2.98	0.00
16	Lu	ModifiedLocality	T32	0.02	3.11	0.05
17	Hull1	CleanVanilla	T1	0.00	0.05	0.00
18	Hull1	CleanVanilla	T32	0.00	0.19	0.00
19	Hull1	ModifiedLocality	T1	0.00	0.10	0.00
20	Hull1	ModifiedLocality	T32	0.00	0.36	0.00
21	Hull2	CleanVanilla	T1	0.00	0.62	0.00
22	Hull2	CleanVanilla	T32	0.00	1.37	0.00
23	Hull2	ModifiedLocality	T1	0.00	0.33	0.00
24	Hull2	ModifiedLocality	T32	0.00	0.55	0.00
25	cg	CleanVanilla	T1	0.00	0.91	0.00
26	cg	CleanVanilla	T32	0.05	2.55	0.13
27	cg	ModifiedLocality	T1	0.00	1.00	0.00
28	cg	ModifiedLocality	T32	0.04	1.29	0.12
}\datatable

\begin{axis}[
    axis lines*=left, ymajorgrids,
    ymin=0,
    ybar stacked,
    bar width=6pt,
    width=6.5in,
    height=4in,
    draw group line={Gp}{Cilksort}{Cilksort}{-4ex}{4pt},
    draw group line={Gp}{Heat}{Heat}{-4ex}{4pt},
    draw group line={Gp}{Strassen}{Strassen}{-4ex}{4pt},
    draw group line={Gp}{Lu}{Lu}{-4ex}{4pt},
    draw group line={Gp}{Hull1}{Hull1}{-4ex}{4pt},
    draw group line={Gp}{Hull2}{Hull2}{-4ex}{4pt},
    draw group line={Gp}{cg}{cg}{-4ex}{4pt},
    draw group line={Type}{CleanVanilla}{C}{-7ex}{4pt},
    draw group line={Type}{ModifiedLocality}{M}{-7ex}{4pt},
    xtick=data,
    xticklabels from table={\datatable}{Cores},
    xticklabel style={rotate=90,xshift=-7ex,anchor=mid east},
]

\addplot table [x=X, y=Work] {\datatable}; \addlegendentry{Work}
\addplot table [x=X, y=Scheduling] {\datatable}; \addlegendentry{Scheduling}
\addplot table [x=X, y=Idle] {\datatable}; \addlegendentry{Idle}
\end{axis}
\end{tikzpicture}
\caption{C = Clean and Vanilla, M = Modified and Locality}
\end{figure}

